Cost-Oriented Load Forecasting

Accurate load prediction is an effective way to reduce power system operation costs. Traditionally, the mean square error (MSE) is a common-used loss function to guide the training of an accurate load forecasting model. However, the MSE loss function is unable to precisely reflect the real costs associated with forecasting errors because the cost caused by forecasting errors in the real power system is probably neither symmetric nor quadratic. To tackle this issue, this paper proposes a generalized cost-oriented load forecasting framework. Specifically, how to obtain a differentiable loss function that reflects real cost and how to integrate the loss function with regression models are studied. The economy and effectiveness of the proposed load forecasting method are verified by the case studies of an optimal dispatch problem that is built on the IEEE 30-bus system and the open load dataset from the Global Energy Forecasting Competition 2012 (GEFCom2012).

==> Cost oriented load forecasting/glossaries.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Make Glossaries                                             %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Required to generate the index for the glossaries.
%\makeglossaries
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                %
%%%%%     Definitions of all glossary entries which will appear in   %
%%%%%     the default (main) glossary.                               %
%%%%%                                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Add all glossary entries to the glossary, even if they have not been
% referenced.
%\glsaddall[types={main}]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                %
%%%%%     Definitions of all acronyms which will appear in the list  %
%%%%%     of acronyms.                                               %
%%%%%                                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newacronym{rbf}{RBF}{Radial Basis Function}
\newacronym{gmm}{GMM}{Gaussian Mixture Model}
\newacronym{em}{EM}{Expectation Maximization}
\newacronym{mle}{MLE}{Maximum Likelihood Estimation}
\newacronym{iid}{i.i.d.}{independently and identically distributed}
%\newacronym{optics}{OPTICS}{Ordering Points To Identify the Clustering Structure}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{svms}{SVMs}{Support Vector Machines}
\newacronym{svr}{SVR}{Support Vector Regression}
%\newacronym{ann}{ANN}{Artificial Neural Network}
%\newacronym{sgd}{SGD}{Stochastic Gradient Descent}
%\newacronym{ffnn}{FFNN}{Feedforward Neural Network}
\newacronym{rf}{RF}{Random Forests}
\newacronym{rfr}{RFR}{Random Forests Regression}
\newacronym{gbrt}{GBRT}{Gradient Boosting Regression Tree}
\newacronym{gbr}{GBR}{Gradient Boosting Regression}
%\newacronym{rnn}{RNN}{Recurrent Neural Network}
%\newacronym{lstm}{LSTM}{Long Short-Term Memory}
%\newacronym{lad}{LAD}{Least Absolute Deviations}
\newacronym{cop}{COP}{Convex Optimization Problem}
\newacronym{lsra}{LSRA}{Least Squares Regression Averaging}
\newacronym{pcr}{PCR}{Principal Component Regression}
\newacronym{flsra}{FLSRA}{Factor Least Squares Regression Averaging}
\newacronym{llsra}{LLSRA}{LASSO Least Squares Regression Averaging}
\newacronym{qra}{QRA}{Quantile Regression Averaging}
\newacronym{fqra}{FQRA}{Factor Quantile Regression Averaging}
\newacronym{lqra}{LQRA}{LASSO Quantile Regression Averaging}
\newacronym{lasso}{LASSO}{Least Absolute Shrinkage and Selection Operator}
\newacronym{lsgbr}{LSGBR}{Least Squares Gradient Boosting Regression}
\newacronym{qgbr}{QGBR}{Quantile Gradient Boosting Regression}
\newacronym{sc}{SC}{Silhouette Coefficient}
\newacronym{chi}{CHI}{Calinski-Harabasz Index}
\newacronym{dbi}{DBI}{Davies-Bouldin Index}
\newacronym{ari}{ARI}{Adjusted Rand Index}
\newacronym{knn}{KNN}{K-Nearest Neighbors}
\newacronym{mae}{MAE}{Mean Absolute Error}
\newacronym{mape}{MAPE}{Mean Absolute Percentage Error}
\newacronym{rmse}{RMSE}{Root Mean Squared Error}
\newacronym{mse}{MSE}{Mean Squared Error}
\newacronym{vif}{VIF}{Variance Inflation Factor}
\newacronym{pi}{PI}{Prediction Interval}
\newacronym{pinc}{PINC}{Prediction Interval Nominal Confidence}
\newacronym{picp}{PICP}{Prediction Interval Coverage Probability}
\newacronym{ace}{ACE}{Average Coverage Error}
\newacronym{pbl}{PBL}{Pinball Loss}
\newacronym{wks}{WKS}{Winkler Score}
\newacronym{smecbts}{SMECBTs}{Smart Metering Electricity Customer Behaviour Trials}
\newacronym{cer}{CER}{Commission for Energy Regulation}




% Add all acronyms to the list of acronyms even if they have not been
% referenced.
%\glsaddall[types={\acronymtype}]

==> Cost oriented load forecasting/preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     preamble.tex                                                %
%%%%%                                                                 %
%%%%% Author:      Michael Muehlberghuber                             %
%%%%% Created:     01.07.2012                                         %
%%%%% Description: This file contains the preamble of the             %
%%%%%              Semester-/Master-Project LaTeX report example.     %
%%%%%                                                                 %
%%%%% History:                                                        %
%%%%%%%%%%%%%%                                                        %
%%%%% 2012/07/01:  *) Created initial version.                        %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Package Loading                                             %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Determines the input encoding.
\usepackage[%
 utf8,
% latin1
]{inputenc}

% ---------------------------------------------------------------------

% Determines the output encoding.
\usepackage[T1]{fontenc}

% ---------------------------------------------------------------------

% Determines language settings.
\usepackage[%
 english    % You may change this to 'ngerman' in order to write a
            % german report.
]{babel}

% ---------------------------------------------------------------------

% Provides image loading.
\usepackage{graphicx}
%\usepackage{subfig}
\usepackage{float}
\graphicspath{{figures/}}
\usepackage{calc}
%\usepackage{svg}

% ---------------------------------------------------------------------

% Provides customization of chapter headings.
\usepackage[%
	Lenny     % Choose a nice layout for chapter headings.
]{fncychap}

% ---------------------------------------------------------------------

% Provides some blindtext.
\usepackage{lipsum}

% ---------------------------------------------------------------------

% Provides stretchable tables.
\usepackage{tabularx}

% ---------------------------------------------------------------------

% Provides some fancy boxes.
\usepackage{fancybox}

% ---------------------------------------------------------------------

% Provides subfigures.
\usepackage{subfig}

% ---------------------------------------------------------------------

% Provides colors in LaTeX.
\usepackage{xcolor}

% ---------------------------------------------------------------------

% Provides conditionals (for titlepage).
\usepackage{xifthen}

% ---------------------------------------------------------------------

% Provides the algorithm environment
\usepackage[ruled, lined, linesnumbered, commentsnumbered, longend]{algorithm2e}

% ---------------------------------------------------------------------

% Provides bold greek math symbols.
\usepackage{bm}
\usepackage{bbm}
\usepackage{amsmath}
\usepackage{amssymb}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\norm}[1]{\left\|#1\right\|}

% ---------------------------------------------------------------------

% Allows to include pdf documents.
\usepackage{pdfpages}
\usepackage{svg}

% ---------------------------------------------------------------------

% Provides nicer tables than the standard tables.
\usepackage{booktabs}
\usepackage{tabu}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{array}
%\usepackage{subcaption}
\makeatletter
\providecommand\phantomcaption{\caption@refstepcounter\@captype}
\makeatother

% ---------------------------------------------------------------------

% Provides simple line spacings.
\usepackage{setspace}

% ---------------------------------------------------------------------

% Provides simple line spacings.
\usepackage{geometry}

% ---------------------------------------------------------------------

% Provides more customizeable captions.
\usepackage{capt-of}

% ---------------------------------------------------------------------

% Provides small table of contents (e.g., for single chapters or the
% appendix).
\usepackage{minitoc}

% ---------------------------------------------------------------------

% Provides a simple command to describe a directory tree.
\usepackage{dirtree}

% ---------------------------------------------------------------------

%%%%%                                                             %%%%%
%%%%% ATTENTION: Loading further packagaes should go in here.     %%%%%
%%%%%                                                             %%%%%

% ---------------------------------------------------------------------

% Provides hyperlinks within your document. Should always be loaded at
% the end.
\usepackage{hyperref}

% ---------------------------------------------------------------------

% Provides multiple glossaries (incl. list acronyms, list of symbols,
% etc.).
\usepackage[%
 toc,              % Add the glossaries to the table of contents.
 acronym,          % Add a list of acronyms.
 section=chapter,  % Show glossary headers as chapters.
 nonumberlist,     % Do not print the page numbers next to glossary
                   % entries.
]{glossaries}

\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Custom Settings                                             %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Do not use sans-serif fonts for all dispositions (chapters,
% sections, etc.)
\setkomafont{disposition}{\normalfont\bfseries}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Custom Macros                                               %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Create an inline command for shell commands.
\newcommand{\shell}[1]{\texttt{#1}}

% Create an enviroment for a shell commands.
\newenvironment{shellenv}%
{\VerbatimEnvironment%
 \begin{Sbox}\begin{minipage}{0.97\textwidth}\begin{Verbatim}%
}%
{\end{Verbatim}\end{minipage}\end{Sbox}%
\setlength{\fboxsep}{6pt}\shadowbox{\TheSbox}}%

% Create an inline command for files.
\newcommand{\file}[1]{\texttt{#1}}

% Create a command for command parameters.
\newcommand{\parameter}[1]{$<$#1$>$}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Titlepage Macros - !!! DO NOT CHANGE !!!                    %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Create a command for missing title page parameters.
\newcommand{\misspar}[1]{\textcolor{red}{\textbf{$<$#1$>$}}}

\makeatletter

% Redefine existing class macros as missing.
\title{\misspar{Specify Title}}%
\author{\misspar{Specify Author}}%
\date{\misspar{Specify Date}}%

% Define a command for setting the semester on the titlepage.
\def\@semester{\misspar{Specify Semester}}%
\newcommand{\setsemester}[1]{\def\@semester{#1}}%
\let\semester\setsemester%
\newcommand{\show@semester}{\@semester}%

% Define a command for setting the type of the report (Master Thesis,
% Semester Project, etc.) on the titlepage.
\def\@reporttype{\misspar{Specify Report Type}}%
\newcommand{\setreporttype}[1]{\def\@reporttype{#1}}%
\let\reporttype\setreporttype%
\newcommand{\show@reporttype}{\@reporttype}%

% Define a command for setting the image path for the image on the
% titlepage.
\def\@titlelogo{}%
\newcommand{\settitlelogo}[1]{\def\@titlelogo{#1}}%
\let\titlelogo\settitlelogo%

% Define a command for setting the image height on the titlepage.
\def\@logoheight{7cm}%
\newcommand{\setlogoheight}[1]{\def\@logoheight{#1}}%
\let\logoheight\setlogoheight%
\newcommand{\show@logoheight}{\@logoheight}%

% Define a command for setting the email on the titlepage.
\def\@email{\misspar{Specify E-Mail}}%
\newcommand{\setemail}[1]{\def\@email{#1}}%
\let\email\setemail%
\newcommand{\show@email}{\@email}%

% Define a command for setting the first supervisor on the titlepage.
\def\@firstsup{\misspar{Specify First Supervisor}}%
\newcommand{\setfirstsup}[1]{\def\@firstsup{#1}}%
\let\firstsup\setfirstsup%
\newcommand{\show@firstsup}{\@firstsup}%

% Define a command for setting the second supervisor on the titlepage.
\def\@secondsup{\misspar{Specify Second Supervisor}}%
\newcommand{\setsecondsup}[1]{\def\@secondsup{#1}}%
\let\secondsup\setsecondsup%
\newcommand{\show@secondsup}{\@secondsup}%

% Define a command for setting the professor on the titlepage.
\def\@professor{\misspar{Specify Professor}}%
\newcommand{\setprofessor}[1]{\def\@professor{#1}}%
\let\professor\setprofessor%
\newcommand{\show@professor}{\@professor}%

% Define a command for setting the margin on the title page.
\def\@titlepagemargin{3cm}%
\newcommand{\settitlepagemargin}[1]{\def\@titlepagemargin{#1}}%
\let\titlepagemargin\settitlepagemargin%
\newcommand{\show@titlepagemargin}{\@titlepagemargin}%

\makeatother


==> glossaries.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Make Glossaries                                             %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Required to generate the index for the glossaries.
%\makeglossaries
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                %
%%%%%     Definitions of all glossary entries which will appear in   %
%%%%%     the default (main) glossary.                               %
%%%%%                                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Add all glossary entries to the glossary, even if they have not been
% referenced.
%\glsaddall[types={main}]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                %
%%%%%     Definitions of all acronyms which will appear in the list  %
%%%%%     of acronyms.                                               %
%%%%%                                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newacronym{rbf}{RBF}{Radial Basis Function}
\newacronym{gmm}{GMM}{Gaussian Mixture Model}
\newacronym{em}{EM}{Expectation Maximization}
\newacronym{mle}{MLE}{Maximum Likelihood Estimation}
\newacronym{iid}{i.i.d.}{independently and identically distributed}
%\newacronym{optics}{OPTICS}{Ordering Points To Identify the Clustering Structure}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{svms}{SVMs}{Support Vector Machines}
\newacronym{svr}{SVR}{Support Vector Regression}
%\newacronym{ann}{ANN}{Artificial Neural Network}
%\newacronym{sgd}{SGD}{Stochastic Gradient Descent}
%\newacronym{ffnn}{FFNN}{Feedforward Neural Network}
\newacronym{rf}{RF}{Random Forests}
\newacronym{rfr}{RFR}{Random Forests Regression}
\newacronym{gbrt}{GBRT}{Gradient Boosting Regression Tree}
\newacronym{gbr}{GBR}{Gradient Boosting Regression}
%\newacronym{rnn}{RNN}{Recurrent Neural Network}
%\newacronym{lstm}{LSTM}{Long Short-Term Memory}
%\newacronym{lad}{LAD}{Least Absolute Deviations}
\newacronym{cop}{COP}{Convex Optimization Problem}
\newacronym{lsra}{LSRA}{Least Squares Regression Averaging}
\newacronym{pcr}{PCR}{Principal Component Regression}
\newacronym{flsra}{FLSRA}{Factor Least Squares Regression Averaging}
\newacronym{llsra}{LLSRA}{LASSO Least Squares Regression Averaging}
\newacronym{qra}{QRA}{Quantile Regression Averaging}
\newacronym{fqra}{FQRA}{Factor Quantile Regression Averaging}
\newacronym{lqra}{LQRA}{LASSO Quantile Regression Averaging}
\newacronym{lasso}{LASSO}{Least Absolute Shrinkage and Selection Operator}
\newacronym{lsgbr}{LSGBR}{Least Squares Gradient Boosting Regression}
\newacronym{qgbr}{QGBR}{Quantile Gradient Boosting Regression}
\newacronym{sc}{SC}{Silhouette Coefficient}
\newacronym{chi}{CHI}{Calinski-Harabasz Index}
\newacronym{dbi}{DBI}{Davies-Bouldin Index}
\newacronym{ari}{ARI}{Adjusted Rand Index}
\newacronym{knn}{KNN}{K-Nearest Neighbors}
\newacronym{mae}{MAE}{Mean Absolute Error}
\newacronym{mape}{MAPE}{Mean Absolute Percentage Error}
\newacronym{rmse}{RMSE}{Root Mean Squared Error}
\newacronym{mse}{MSE}{Mean Squared Error}
\newacronym{vif}{VIF}{Variance Inflation Factor}
\newacronym{pi}{PI}{Prediction Interval}
\newacronym{pinc}{PINC}{Prediction Interval Nominal Confidence}
\newacronym{picp}{PICP}{Prediction Interval Coverage Probability}
\newacronym{ace}{ACE}{Average Coverage Error}
\newacronym{pbl}{PBL}{Pinball Loss}
\newacronym{wks}{WKS}{Winkler Score}
\newacronym{smecbts}{SMECBTs}{Smart Metering Electricity Customer Behaviour Trials}
\newacronym{cer}{CER}{Commission for Energy Regulation}




% Add all acronyms to the list of acronyms even if they have not been
% referenced.
%\glsaddall[types={\acronymtype}]

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     preamble.tex                                                %
%%%%%                                                                 %
%%%%% Author:      Michael Muehlberghuber                             %
%%%%% Created:     01.07.2012                                         %
%%%%% Description: This file contains the preamble of the             %
%%%%%              Semester-/Master-Project LaTeX report example.     %
%%%%%                                                                 %
%%%%% History:                                                        %
%%%%%%%%%%%%%%                                                        %
%%%%% 2012/07/01:  *) Created initial version.                        %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Package Loading                                             %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Determines the input encoding.
\usepackage[%
 utf8,
% latin1
]{inputenc}

% ---------------------------------------------------------------------

% Determines the output encoding.
\usepackage[T1]{fontenc}

% ---------------------------------------------------------------------

% Determines language settings.
\usepackage[%
 english    % You may change this to 'ngerman' in order to write a
            % german report.
]{babel}

% ---------------------------------------------------------------------

% Provides image loading.
\usepackage{graphicx}
%\usepackage{subfig}
\usepackage{float}
\graphicspath{{figures/}}
\usepackage{calc}
%\usepackage{svg}

% ---------------------------------------------------------------------

% Provides customization of chapter headings.
\usepackage[%
	Lenny     % Choose a nice layout for chapter headings.
]{fncychap}

% ---------------------------------------------------------------------

% Provides some blindtext.
\usepackage{lipsum}

% ---------------------------------------------------------------------

% Provides stretchable tables.
\usepackage{tabularx}

% ---------------------------------------------------------------------

% Provides some fancy boxes.
\usepackage{fancybox}

% ---------------------------------------------------------------------

% Provides subfigures.
\usepackage{subfig}

% ---------------------------------------------------------------------

% Provides colors in LaTeX.
\usepackage{xcolor}

% ---------------------------------------------------------------------

% Provides conditionals (for titlepage).
\usepackage{xifthen}

% ---------------------------------------------------------------------

% Provides the algorithm environment
\usepackage[ruled, lined, linesnumbered, commentsnumbered, longend]{algorithm2e}

% ---------------------------------------------------------------------

% Provides bold greek math symbols.
\usepackage{bm}
\usepackage{bbm}
\usepackage{amsmath}
\usepackage{amssymb}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\norm}[1]{\left\|#1\right\|}

% ---------------------------------------------------------------------

% Allows to include pdf documents.
\usepackage{pdfpages}
\usepackage{svg}

% ---------------------------------------------------------------------

% Provides nicer tables than the standard tables.
\usepackage{booktabs}
\usepackage{tabu}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{array}
%\usepackage{subcaption}
\makeatletter
\providecommand\phantomcaption{\caption@refstepcounter\@captype}
\makeatother

% ---------------------------------------------------------------------

% Provides simple line spacings.
\usepackage{setspace}

% ---------------------------------------------------------------------

% Provides simple line spacings.
\usepackage{geometry}

% ---------------------------------------------------------------------

% Provides more customizeable captions.
\usepackage{capt-of}

% ---------------------------------------------------------------------

% Provides small table of contents (e.g., for single chapters or the
% appendix).
\usepackage{minitoc}

% ---------------------------------------------------------------------

% Provides a simple command to describe a directory tree.
\usepackage{dirtree}

% ---------------------------------------------------------------------

%%%%%                                                             %%%%%
%%%%% ATTENTION: Loading further packagaes should go in here.     %%%%%
%%%%%                                                             %%%%%

% ---------------------------------------------------------------------

% Provides hyperlinks within your document. Should always be loaded at
% the end.
\usepackage{hyperref}

% ---------------------------------------------------------------------

% Provides multiple glossaries (incl. list acronyms, list of symbols,
% etc.).
\usepackage[%
 toc,              % Add the glossaries to the table of contents.
 acronym,          % Add a list of acronyms.
 section=chapter,  % Show glossary headers as chapters.
 nonumberlist,     % Do not print the page numbers next to glossary
                   % entries.
]{glossaries}

\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Custom Settings                                             %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Do not use sans-serif fonts for all dispositions (chapters,
% sections, etc.)
\setkomafont{disposition}{\normalfont\bfseries}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Custom Macros                                               %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Create an inline command for shell commands.
\newcommand{\shell}[1]{\texttt{#1}}

% Create an enviroment for a shell commands.
\newenvironment{shellenv}%
{\VerbatimEnvironment%
 \begin{Sbox}\begin{minipage}{0.97\textwidth}\begin{Verbatim}%
}%
{\end{Verbatim}\end{minipage}\end{Sbox}%
\setlength{\fboxsep}{6pt}\shadowbox{\TheSbox}}%

% Create an inline command for files.
\newcommand{\file}[1]{\texttt{#1}}

% Create a command for command parameters.
\newcommand{\parameter}[1]{$<$#1$>$}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%                                                                 %
%%%%%     Titlepage Macros - !!! DO NOT CHANGE !!!                    %
%%%%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Create a command for missing title page parameters.
\newcommand{\misspar}[1]{\textcolor{red}{\textbf{$<$#1$>$}}}

\makeatletter

% Redefine existing class macros as missing.
\title{\misspar{Specify Title}}%
\author{\misspar{Specify Author}}%
\date{\misspar{Specify Date}}%

% Define a command for setting the semester on the titlepage.
\def\@semester{\misspar{Specify Semester}}%
\newcommand{\setsemester}[1]{\def\@semester{#1}}%
\let\semester\setsemester%
\newcommand{\show@semester}{\@semester}%

% Define a command for setting the type of the report (Master Thesis,
% Semester Project, etc.) on the titlepage.
\def\@reporttype{\misspar{Specify Report Type}}%
\newcommand{\setreporttype}[1]{\def\@reporttype{#1}}%
\let\reporttype\setreporttype%
\newcommand{\show@reporttype}{\@reporttype}%

% Define a command for setting the image path for the image on the
% titlepage.
\def\@titlelogo{}%
\newcommand{\settitlelogo}[1]{\def\@titlelogo{#1}}%
\let\titlelogo\settitlelogo%

% Define a command for setting the image height on the titlepage.
\def\@logoheight{7cm}%
\newcommand{\setlogoheight}[1]{\def\@logoheight{#1}}%
\let\logoheight\setlogoheight%
\newcommand{\show@logoheight}{\@logoheight}%

% Define a command for setting the email on the titlepage.
\def\@email{\misspar{Specify E-Mail}}%
\newcommand{\setemail}[1]{\def\@email{#1}}%
\let\email\setemail%
\newcommand{\show@email}{\@email}%

% Define a command for setting the first supervisor on the titlepage.
\def\@firstsup{\misspar{Specify First Supervisor}}%
\newcommand{\setfirstsup}[1]{\def\@firstsup{#1}}%
\let\firstsup\setfirstsup%
\newcommand{\show@firstsup}{\@firstsup}%

% Define a command for setting the second supervisor on the titlepage.
\def\@secondsup{\misspar{Specify Second Supervisor}}%
\newcommand{\setsecondsup}[1]{\def\@secondsup{#1}}%
\let\secondsup\setsecondsup%
\newcommand{\show@secondsup}{\@secondsup}%

% Define a command for setting the professor on the titlepage.
\def\@professor{\misspar{Specify Professor}}%
\newcommand{\setprofessor}[1]{\def\@professor{#1}}%
\let\professor\setprofessor%
\newcommand{\show@professor}{\@professor}%

% Define a command for setting the margin on the title page.
\def\@titlepagemargin{3cm}%
\newcommand{\settitlepagemargin}[1]{\def\@titlepagemargin{#1}}%
\let\titlepagemargin\settitlepagemargin%
\newcommand{\show@titlepagemargin}{\@titlepagemargin}%

\makeatother

